Optimal Good-Case Latency for Sleepy Consensus

In the context of Byzantine consensus problems such as Byzantine broadcast (BB) and Byzantine agreement (BA), the good-case setting aims to study the minimal possible latency of a BB or BA protocol under certain favorable conditions, namely the designated leader being correct (for BB), or all parties having the same input value (for BA). We provide a full characterization of the feasibility and impossibility of good-case latency, for both BA and BB, in the synchronous sleepy model. Surprisingly to us, we find irrational resilience thresholds emerging: 2-round good-case BB is possible if and only if at all times, at least $\frac{1}{\varphi} \approx 0.618$ fraction of the active parties are correct, where $\varphi = \frac{1+\sqrt{5}}{2} \approx 1.618$ is the golden ratio; 1-round good-case BA is possible if and only if at least $\frac{1}{\sqrt{2}} \approx 0.707$ fraction of the active parties are correct.

==> lib/defer.tex <==
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\RequirePackage{expl3}
\RequirePackage{scontents}


%
%
%
\ExplSyntaxOn

%
%
%
\cs_new_protected:Npn \defer_new_group:nn #1 #2 {
  %
  \bool_if_exist:cF { l__defer_#1 _bool } { \bool_new:c { l__defer_#1 _bool } }
  %
  \tl_set:Nx \l_tmpa_tl { \tl_lower_case:n {#2} }
  %
  \str_if_eq:VnTF \l_tmpa_tl {deferred}
    { \bool_set_true:c  { l__defer_#1 _bool } }
    { \bool_set_false:c { l__defer_#1 _bool } }
}


%
%
%

%
%
\NewDocumentCommand{\newdefergroup}{m O{deferred}}{
  \defer_new_group:nn {#1}{#2}
}

%
%
\NewDocumentEnvironment{ifdeferred}{m +b}{%
  \bool_if:cT { l__defer_#1 _bool } { #2 }%
}{}

%
%
\NewDocumentEnvironment{ifnotdeferred}{m +b}{%
  \bool_if:cF { l__defer_#1 _bool } { #2 }%
}{}

%
%
%
\NewDocumentEnvironment{defer}{m +b}{%
  \bool_if:cTF { l__defer_#1 _bool }{%
    %
    \Scontents[store-cmd=defer@#1,print-cmd=false]{#2}%
  }{%
    %
    #2%
  }%
}{}

%
%
\NewDocumentCommand{\printdefergroup}{m}{%
  %
  \foreachsc{defer@#1}%
}

\ExplSyntaxOff

%
%
%

%
%
%
%
\NewDocumentCommand{\deferredproof}{m m}{%
  \begin{ifdeferred}{#1}%
    Proof of \cref{#2} is deferred to \cref{sec:deferred-#1}.%
  \end{ifdeferred}%
}

%
%
%
\NewDocumentCommand{\deferredsection}{m m}{%
  \begin{ifdeferred}{#1}%
    \section{#2}%
    \label{sec:deferred-#1}%
    \printdefergroup{#1}%
  \end{ifdeferred}%
}

